Towards Human-Compatible XAI: Explaining Data Differentials with Concept Induction over Background Knowledge

Concept induction, which is based on formal logical reasoning over description logics, has been used in ontology engineering in order to create ontology (TBox) axioms from the base data (ABox) graph. In this paper, we show that it can also be used to explain data differentials, for example in the context of Explainable AI (XAI), and we show that it can in fact be done in a way that is meaningful to a human observer. Our approach utilizes a large class hierarchy, curated from the Wikipedia category hierarchy, as background knowledge.

==> cut-text-ignore.tex <==



In the first experiment the quality of ECII-generated explanations was (subjectively) judged by human participants, by comparison with human- and random-generated explanations. In the second experiment we aim to obtain an objective measure of the quality of ECII's explanations. 

The goal of the second experiment was to test whether the ECII explanations helped human participants identify the errors made by a machine learning classifier (a logistic regression model). 

4.1. Hypothesis

We hypothesize that 

4.2. Method

Stimuli

Annotated images from Google Open Images database \textcolor{red}{add reference} were selected for this study. The following themes were used for selection: kitchens, bedrooms, dinning rooms, offices, parking lots, workshops, parks, pantries, classrooms, and public libraries.   

The annotations are human generated, thus noisy. Some manual curation was done as part of the image selection process    \textcolor{red}{Srikanth, please add some detail here: why and how we did it}

Images were classified by the logistic regression model in four categories: true positives (TP), true negatives (TN), false positives (FP), and false negatives (FN). 

\textcolor{red}{add detail here about how explanations were generated. what metrics to use: precision, F1, etc. We decided to use F1 as a trade-off between precision and recall. We decided to pool the first 10 or 15 explanations and take the unique concepts from that pool.} 


Experimental set-up on Mechanical Turk

Experimental Design

Conditions: 

Between-subjects

Explanandum (i.e., which image set is explained): correct vs error.

In the explanandum-correct condition, the ECII algorithm generates an explanation for the correct image set - TP or TN. 

In the explanandum-error condition, the ECII algorithm generates an explanation for the error image set - FP or FN. 

Within-subjects

Error type \textcolor{red}{IJ: I am assuming this will be done within-subjects}: FP and FN

In the FN condition, the image sets presented to the participants are from the TP and FN categories. 

In the FP condition, the image sets presented to the participants are from the FP and TN categories. 

Explanation source \textcolor{red}{IJ: I am assuming this will also be done within-subjects}: ECII, human (gold standard), random, and no explanation \textcolor{red}{IJ: the latter will need to be matched in terms of interface info and participant action to the other conditions} 
\textcolor{red}{IJ: Alternatively, the no-explanation condition could be integrated with all the other conditions as a pretest/baseline measure. Josh has some concerns that this might bias participants to stick with their initial no-explanation response. I am less concerned because the bias (if there is one) will be spread evenly across the other conditions. I also think the benefit of knowing the non-assisted accuracy outweighs the risk of a bias. Note that this way we obtain a noise-free measure of non-assisted accuracy because the variability across subjects and items is automatically controlled for.}

\textcolor{red}{IJ: For completeness, I suggest another condition: the set-difference explanation. This will be an explanation in terms of the actual annotations, thus missing the concept induction part.}

Procedure

The participants were told that an AI algorithm tried to identify images with a particular theme (e.g., kitchens) in a larger image database. 

Then, participants were shown two sets of images sampled from those that were generated by the logistic regression model. One of the two sets was an error set (FP or FN). The participant's task was to identify the error set. Thus, if the two sets of images shown to the participant were sampled from the TP and FN categories, the participant had to identify the FN set as the error set; if the two sets of images shown to the participant were sampled from the FP and TN categories, the participant had to identify the FP set as the error set.  


4.3. Results

\textcolor{red}{IJ: how do I insert graphs? Please insert a graph so I can see an example. PH: see Figure \ref{imagelabel2}. Can also be double-column.}

\begin{figure}[tb]
\includegraphics[width=\columnwidth]{daselab-shamrock.png}
\caption{Image caption}\label{imagelabel2}
\end{figure}

4.4. Discussion of the results of Experiment 2

A question that we have not addressed directly in this study is how humans detect the error set. Do they notice that the error images (include) exclude certain objects that the correct images (do not) contain?  


